Room Temperature Hydrogen Atom Scattering Experiments Are Not a Sufficient Benchmark to Validate Electronic Friction Theory

In the dynamics of atoms and molecules at metal surfaces, electron-hole pair excitations can play a crucial role. In the case of hyperthermal hydrogen atom scattering, they lead to nonadiabatic energy loss and highly inelastic scattering. Molecular dynamics with electronic friction simulations where friction is computed under an isotropic homogeneous electron gas approximation have previously shown good agreement with measured kinetic energy loss distributions, suggesting that this level of theoretical description is sufficient to describe nonadiabatic effects of atomic scattering. In this work, we show that similar agreement with room temperature experiments can also be achieved with friction derived from density functional theory linear response calculations. The apparent agreement of the homogeneous electron gas approximation with experiment arises from a fortuitous cancellation of errors where friction is overestimated close to the surface and the spin transition is neglected. Only for scattering at low temperatures can both approximations be distinguished and differences rationalised in terms of the number of bounces of the atom on the surface. We identify the signatures of nonadiabatic energy loss of different levels of theory, which future low-temperature scattering experiments will be able to measure.

==> jpcl_introduction.tex <==
The scattering of hyperthermal hydrogen atoms with metal surfaces is a well-studied phenomenon, known to cause substantial energy transfer to the surface~\cite{bunermann_electron-hole_2015}. At room temperature, the energy loss distributions (ELDs) of scattering hydrogen atoms are broad, lacking distinct features with only subtle differences between metal surfaces~\cite{dorenkamp_hydrogen_2018, hertl_electronically_2022}. Classical molecular dynamics (MD) simulations underestimate this energy transfer because they do not account for nonadiabatic effects during the dynamics and the excitation of electron-hole pairs (EHPs) in the metal.\cite{bunermann_electron-hole_2015, janke_accurate_2015} To address this shortcoming, several simulation methods have been developed, among which molecular dynamics with electronic friction (MDEF) stands out as a practically feasible approach. MDEF has been applied to the dynamics of atoms~\cite{janke_accurate_2015,askerka_role_2016} and molecules~\cite{maurer_mode_2017,galparsoro_hydrogen_2016,spiering_testing_2018, zhang_hot-electron_2019, box_determining_2021} at metal surfaces, including under the influence of laser pulses.~\cite{fuchsel_dissipative_2011,scholz_femtosecond-laser_2016} Theoretical studies applying MDEF simulations to H atom scattering~\cite{Janke_PhD_2016,kandratsenka_unified_2018,martin_h_2022} were able to link scattering events with low energy loss to hydrogen atoms that primarily undergo a single bounce on the surface, while events that exhibit high energy losses are associated with atoms that experience multiple bounces.

MDEF simulates the dynamics on the ground state adiabatic potential energy surface while introducing a drag force on the nuclear motion, that accounts for the energy transfer to electron-hole pair excitations.\cite{headgordon_molecular_1995} Remarkably, MDEF simulations have successfully reproduced the ELDs for hydrogen atom scattering from a variety of metal surfaces.\cite{janke_accurate_2015,dorenkamp_hydrogen_2018, hertl_electronically_2022} This success, however, is puzzling for several reasons. 

Firstly, in the context of hydrogen atom scattering from a metal surface, a strong nonadiabatic effect arises due to the screening of the unpaired spin of the hydrogen atom in close vicinity of the metal surface. Such pronounced nonadiabatic effects are typically beyond the scope of electronic friction.\cite{mizielinski_electronic_2005} Indeed, it was previously shown that electronic friction in the Markov (quasi-adiabatic) approximation gives rise to a sudden rise in stopping power at the spin transition geometry.\cite{ mizielinski_electronic_2005, trail_electronhole_2003} While this effect is "broadened out" in nonadiabatic mean-field (Ehrenfest) dynamics due to memory  effects,~\cite{lindenblatt_ab_2006} its contribution to the energy loss is similar and significant in both cases.~\cite{mizielinski_newnsanderson_2008} Previous MDEF studies of hyperthermal hydrogen scattering \cite{janke_accurate_2015,dorenkamp_hydrogen_2018, hertl_electronically_2022} have effectively ignored this spin transition by employing the local-density friction approximation (LDFA), which evaluates electronic friction under a homogeneous electron gas approximation and neglects the electronic structure and spin state of the adsorbate. As a result, these studies are expected to underestimate energy loss by overlooking this effect. 

Secondly, while the magnitude of electronic friction from LDFA and time-dependent perturbation theory align for the homogeneous electron gas~\cite{hellsing_electronic_1984}, the validity of LDFA for interacting densities has been questioned\cite{luntz_comment_2009}. 
LDFA data presented in several works\cite{luntz_comment_2009,askerka_role_2016,spiering_testing_2018} involving hydrogen atoms and molecules interacting with metal surfaces overestimate friction when compared to friction predictions based on density functional theory (DFT) linear response calculations, sometimes referred to as orbital-dependent friction (ODF). This overestimation of friction close to the surface results in an underestimation of the vibrational hydrogen atom relaxation time on surfaces. For example, reported hydrogen relaxation times 
by LDFA for Pd(100) (0.2 ps)\cite{blanco-rey_electronic_2014}, Ru(0001) (0.2 ps)\cite{fuchsel_dissipative_2011}, and Pb(111) (0.3 ps)\cite{saalfrank_vibrational_2014} are a factor of 3-4 faster than experimental measurements for hydrogen atom relaxation on Pt(111) (0.8 ps)\cite{palecek_characterization_2018} and Cu(111) ( 0.7 ps)\cite{lamont_dynamics_1995}. Such an overestimation of friction should also affect the predicted ELDs of scattered H atoms.

In this work, we simulate hyperthermal hydrogen scattering on Pt(111) for which experiments were previously reported.~\cite{dorenkamp_hydrogen_2018,lecroart_adsorbate_2021} We perform MDEF simulations with two electronic friction tensor models based on LDFA and full DFT linear response calculations, i.e., ODF.~\cite{maurer_ab_2016,box_ab_2023}  The two models exhibit very different configuration-dependence of friction, yet both predict room temperature ELDs that are statistically indistinguishable from the experiment. DFT-based electronic friction predicts lower energy loss close to the surface than LDFA, which is in better agreement with time-resolved spectroscopy measurements, but only matches the experimental ELD if the spin transition is included. Simulations of low-temperature ELDs, however, reveal clear differences that arise from the specific features of the two friction profiles.
